Nuclear modification factor for gluon jets

It is shown that the nuclear modification factor can be smaller that unity for jet production at small $x$ and at large transverse momentum without any violation of the factorization theorem and the initial state effects is able to explain the nuclear modification factor of the order of the one measured by ATLAS. In other word, initial state effects are able to describe the jet quenching for the gluon jet production.

==> NMFjet-ref.tex <==
\begin{thebibliography}{99}

\bibitem{ATLAS}
ATLAS collaboration: {\it ``Centrality dependence of Jet Yields and Jet Fragmentation in Lead-Lead
Collisions at $\sqrt{s}_{NN} = 2.76 TeV$ with the ATLAS detector at the LHC"}, ATLAS-CONF-2011-075.
\bibitem{FT1}
J.~C.~Collins, D.~E.~Soper and G.~F.~Sterman,
  %``Factorization of Hard Processes in QCD,''
  Adv.\ Ser.\ Direct.\ High Energy Phys.\  {\bf 5} (1988) 1
  [arXiv:hep-ph/0409313].
  %%CITATION = 00319,5,1;%%

\bibitem{FT2}
J.~C.~Collins, D.~E.~Soper and G.~F.~Sterman,
  %``Soft Gluons and Factorization,''
  Nucl.\ Phys.\  B {\bf 308} (1988) 833.
  %%CITATION = NUPHA,B308,833;%%
\bibitem{FT3}
 G.~T.~Bodwin,
  %``Factorization Of The Drell-Yan Cross-Section In Perturbation Theory,''
  Phys.\ Rev.\  D {\bf 31} (1985) 2616
  [Erratum-ibid.\  D {\bf 34} (1986) 3932]
  [Phys.\ Rev.\  D {\bf 34} (1986) 3932].
  %%CITATION = PHRVA,D34,3932;%%

\bibitem{FT4}
 J.~C.~Collins, D.~E.~Soper and G.~F.~Sterman,
  %``Factorization For Short Distance Hadron - Hadron Scattering,''
  Nucl.\ Phys.\  B {\bf 261} (1985) 104.
  %%CITATION = NUPHA,B261,104;%%


\bibitem{KTF1}
 S.~Catani, M.~Ciafaloni and F.~Hautmann,
  %``High-energy factorization and small x heavy flavor production,''
  Nucl.\ Phys.\  B {\bf 366} (1991) 135.
  %%CITATION = NUPHA,B366,135;%%
\bibitem{KTF2}
S.~Catani, M.~Ciafaloni and F.~Hautmann,
  %``Leptoproduction of heavy flavor at high energies,''
  Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 29A} (1992) 182.
  %%CITATION = NUPHZ,29A,182;%%
\bibitem{KTF3}
J.~C.~Collins and R.~K.~Ellis,
  %``Heavy quark production in very high-energy hadron collisions,''
  Nucl.\ Phys.\  B {\bf 360} (1991) 3.
\bibitem{KTF4}
E.~M.~Levin, M.~G.~Ryskin, Yu.~M.~Shabelski and A.~G.~Shuvaev,
  %``Heavy Quark Production In Semihard Nucleon Interactions,''
  Sov.\ J.\ Nucl.\ Phys.\  {\bf 53} (1991) 657
  [Yad.\ Fiz.\  {\bf 53} (1991) 1059].
  %%CITATION = YAFIA,53,1059;%%

\bibitem{DGLAP}
 V. N. Gribov and L. N. Lipatov,  Sov. J. Nucl. Phys {\bf 15} (1972)
                438;\\
 G. Altarelli and G. Parisi, Nucl. Phys. {\bf B 126} (1977) 298; \\
Yu. l. Dokshitser, Sov. Phys. JETP {\bf 46}  (1977) 641.

\bibitem{BFKL}
 E. A. Kuraev, L. N. Lipatov, and F. S. Fadin,  Sov. Phys. JETP
                {\bf 45} (1977) 199 ; \\
Ya. Ya. Balitsky and L. N. Lipatov,
                Sov. J. Nucl. Phys.\, {\bf 28} (1978) 22 .


\bibitem{GLR}
L. V. Gribov, E. M. Levin and M. G. Ryskin, 
Phys. Rep. {\bf 100} (1983) 1. 

\bibitem{MUSH}
  A.~H.~Mueller, A.~I.~Shoshi,
  %``Small x physics beyond the Kovchegov equation,''
  Nucl.\ Phys.\  {\bf B692}, 175-208 (2004).
  [hep-ph/0402193].


\bibitem{KLM}
  D.~Kharzeev, E.~Levin, L.~McLerran,
  %``Parton saturation and N(part) scaling of semihard processes in QCD,''
  Phys.\ Lett.\  {\bf B561 } (2003)  93-101.
  [hep-ph/0210332
\bibitem{MV}
L. McLerran and R. Venugopalan, 
Phys. Rev. {\bf D49} (1994) 2233, 3352; {\bf D50} (1994) 2225; 
{\bf D53} (1996) 458;\\ {\bf D59} (1999) 09400. 

  \bibitem{GS}
   J.~Bartels and E.~Levin,
  %``Solutions To The Gribov-Levin-Ryskin Equation In The Nonperturbative
  %Region,''
  Nucl.\ Phys.\  B {\bf 387} (1992) 617;\,\,\,
   A.~M.~Stasto, K.~J.~Golec-Biernat and J.~Kwiecinski,
  %``Geometric scaling for the total gamma* p cross-section in the low x
  %region,''
  Phys.\ Rev.\ Lett.\  {\bf 86} (2001) 596
  [arXiv:hep-ph/0007192];\,\,\, E.~Iancu, K.~Itakura and L.~McLerran,
  %``Geometric scaling above the saturation scale,''
  Nucl.\ Phys.\  A {\bf 708} (2002) 327
  [arXiv:hep-ph/0203137].
  %%CITATION = NUPHA,A708,327;%%

  %%CITATION = PRLTA,86,596;%%

  \bibitem{KTINC}
   Y.~V.~Kovchegov and K.~Tuchin,
  %``Inclusive gluon production in DIS at high parton density,''
  Phys.\ Rev.\  D {\bf 65} (2002) 074026
  [arXiv:hep-ph/0111362].
  %%CITATION = PHRVA,D65,074026;%%

\bibitem{DISSTR}
 See  Durham database:
http://hepdata.cedar.ac.uk/pdfs





\bibitem{KLN}
D.~Kharzeev, E.~Levin and M.~Nardi,
  %``QCD saturation and deuteron nucleus collisions,''
  Nucl.\ Phys.\  A {\bf 730} (2004) 448
  [Erratum-ibid.\  A {\bf 743} (2004) 329]
  [arXiv:hep-ph/0212316];\,\
%``The onset of classical QCD dynamics in relativistic heavy ion
  %collisions,''
  Phys.\ Rev.\  C {\bf 71} (2005) 054903
  [arXiv:hep-ph/0111315];\,\, D.~Kharzeev and E.~Levin,
  %``Manifestations of high density QCD in the first RHIC data,''
  Phys.\ Lett.\  B {\bf 523} (2001) 79
  [arXiv:nucl-th/0108006];\,\,\, D.~Kharzeev and M.~Nardi,
  %``Hadron production in nuclear collisions at RHIC and high density QCD,''
  Phys.\ Lett.\  B {\bf 507} (2001) 121
  [arXiv:nucl-th/0012025];\,\,
  D.~Kharzeev, E.~Levin and M.~Nardi,
  %``Color glass condensate at the LHC: Hadron multiplicities in p p, p A  and A
  %A collisions,''
  Nucl.\ Phys.\  A {\bf 747} (2005) 609
  [arXiv:hep-ph/0408050].;\,\,\,
  %%CITATION = NUPHA,A747,609;%%
A.~Dumitru, D.~E.~Kharzeev, E.~M.~Levin and Y.~Nara,
  {\it ``Gluon saturation in $pA$ collisions at the LHC: KLN model predictions for hadron multiplicities,''}
  arXiv:1111.3031 [hep-ph].
  %%CITATION = ARXIV:1111.3031;%%,

  %%CITATION = PHLTA,B507,121;%%
  %%CITATION = PHLTA,B523,79;%%
  %%CITATION = PHRVA,C71,054903;%%
  %%CITATION = NUPHA,A730,448;%%
\bibitem{EKL}
R.~K.~Ellis, Z.~Kunszt and E.~M.~Levin,
  %``The Evolution of parton distributions at small x,''
  Nucl.\ Phys.\ B {\bf 420}, 517 (1994)
  [Erratum-ibid.\ B {\bf 433}, 498 (1995)].
  %%CITATION = NUPHA,B420,517;%%








\end{thebibliography}




\end{document}


